Comparison of remote experiments using crowdsourcing and laboratory experiments on speech intelligibility

Many subjective experiments have been performed to develop objective speech intelligibility measures, but the novel coronavirus outbreak has made it very difficult to conduct experiments in a laboratory. One solution is to perform remote testing using crowdsourcing; however, because we cannot control the listening conditions, it is unclear whether the results are entirely reliable. In this study, we compared speech intelligibility scores obtained in remote and laboratory experiments. The results showed that the mean and standard deviation (SD) of the remote experiments' speech reception threshold (SRT) were higher than those of the laboratory experiments. However, the variance in the SRTs across the speech-enhancement conditions revealed similarities, implying that remote testing results may be as useful as laboratory experiments to develop an objective measure. We also show that the practice session scores correlate with the SRT values. This is a priori information before performing the main tests and would be useful for data screening to reduce the variability of the SRT distribution.

==> Previous/memo.tex <==


% \ref{sec:exp_Crowd}節で説明した遠隔実験での音声了解度を算出し、\ref{sec:exp_Lab}節の防音室での実験結果\cite{Ohashi2018Babble, Iwaki2019Onatsu}と比較を行った。



In general, subjective quality measures require that:
1. there are enough listening subjects of sufficient diversity to deliver statistically significant results;
2. experiments are conducted in a controlled environment with specific acoustic characteristics and equipment;
3. every subject receives the same instructions and stimuli.

In this paper, we propose a class of subjective listening tests which are obtained by relaxing requirement (2) listed above. Instead of running a MOS test in a controlled environment, we outsource this task to workers from an internet crowd, obtaining a measure we call crowdMOS. Several companies provide elements to help facilitate or intermediate this crowdsourcing, with the most famous probably being Amazon Mechanical Turk [7], which we use in our approach. Recruited workers conduct listening experiments at their leisure, us- ing their own hardware. They are typically non-experts drawn from a pool of hundreds of thousands of individuals distributed around the world. Thus, a crowdMOS study can easily have a much larger and more diverse pool than a traditional MOS study, at a significantly lower cost. On the other hand, crowdMOS has to deal with the work- ers’ lack of supervision and uncontrolled environment. Even though we provide financial incentive for workers to deliver high quality re- sults, they have no obligation to do so. Thus, we propose a screening process to detect and discard inaccurate or malicious submissions.


% xxxx xxxx xxxx xxxx xxxx xxxx xxxx xxxx xxxx xxxx xxxx xxxx xxxx xxxx 
%ここでは、実際に実験してみて、何が実験結果に影響を及ぼすか調査。

%参考
% remote : Amazon AMTをつかって、speech quality やpreference of TTS のものが多い。
% しかし、speech intellibilityに関する報告はrelatively 少ない。

% Massive data を集めるには有利。しかし実験統制することや、hearing level等を的確に把握することは困難。

%ここでは、実際に実験してみて、何が実験結果に影響を及ぼすか調査。
%この結果、練習問題の成績が、variabilityを減らすデータ削減に良い指標(？)/有効であることがわかった。


%%--------------------------------------------------------------
%\subsubsection{心理物理曲線}
%\label{sec:ExpResult}
%%--------------------------------------------------------------
%実験参加者29名分の回答データから、心理物理曲線を各音声強調処理条件ごとに算出した。図\ref{fig:ExpAYama20_Sbj29}上図にSNRの関数とした参加者平均の心理物理曲線と標準偏差を示す。これに対して、図\ref{fig:ExpLab_KY17}上図に防音室実験\cite{Ohashi2018Babble}の結果を、図\ref{fig:ExpLabLowSPL_RI18}上図に防音室音圧低減実験\cite{Iwaki2019Onatsu}の結果を示す。お互いの関係がわかるように、背景に薄く別の実験の心理物理曲線も描いてある。これを見ると、今回の遠隔実験の平均了解度は、防音室実験にくらべて全体的にやや了解度が低くく、標準偏差がやや大きいことがわかる。しかし、3者の標準偏差は重なっており、差異は大きくない。


%\subsection{遠隔聴取実験の条件}　% 実験機材・実験参加者・実験手法
\label{sec:exp_Crowd}
%%--------------------------------------------------------------
%遠隔実験では、クラウドソーシング(Lancers\cite{Lancers})のタスクの時間制限(120分)を勘案し、強調信号処理の組み合わせを、\{``Unprocessed'', ``SS10''\}と\{``VTS00'',``VTS02''\}の2組に分割し、それぞれ異なる200単語を用いた。単語の再生順序はランダム化したが、Webページの制約から、実験参加者ごとに再生される単語を変えることは行わなかった。この2分割した実験は、数日あけて順番に実施した。前記のように1実験は2$\sim$3日で終了する。

%音声提示条件は通常音圧($L_A_{eq}=63 $ dB)の防音室実験\cite{Ohashi2018Babble, yamamoto2020gedi}とほぼ同様である。SNRは-6\,dBから+6\,dBの3\,dB刻みの5段階に設定し、音声提示毎に無音4秒間の回答時間がある。

%1実験あたりの参加者はLancersに登録している30名で、実験タスク公開時から早い者順に参加した。事前に年齢・性別・聴力レベル・使用音響機材・学歴等の参加条件の統制は行なわなかった。条件を変えて2回実験を行い、2回とも参加したのは16名であったので、全部で44名である。参加者は、今回の遠隔実験用に制作したWebページ\cite{ExpSpIntel}(付録A参照)に従って実験を遂行した。各自のヘッドホンやイヤホンで「聞き取りやすい」音の大きさに設定した。また、事前に印刷した回答用紙に手書きで聞き取った音声をひらがなで回答を記入するように指示された。1セッション10単語の聞き取りが終了した時点で、記入した手書き文字を本人がWebページの入力欄にタイプインし、それを20セッション分繰り返した。

%参加者は、Webページ\cite{ExpSpIntel}(付録A)の遷移に従って、実験を実施した。
%、実験説明書を読み同意ボタン押す。すると別ページに遷移するので、もう一度確認ボタンを押すことにより実験に参加した。これは間違いを予防するためである。

% どこかで練習セッションについていれたい
% \color{red}

%このような実験に初めて参加する人にタスクを理解してもらうために、練習セッションを設けた。本番と同じ形式にして1セッション10単語としたが、わかりやすいように、高親密度単語の音声強調処理無条件``Unprocessed''のみとし、SNRを0\,dBから+6\,dBの3\,dB刻みの3段階とした。




%今回の遠隔実験においては、参加者がタイプインしたデータに加えて、手書きした回答用紙のスキャンデータも提出してもらった。これら全てが揃ってタスク完了とし、謝金を支払われるようにタスク設定をした。
%回答確認のためと、音声を聞かずでたらめに回答することがないようにするためである。

%まず、タイプインデータに関して、指示どおり4モーラとなっているかプログラムを実行して確認し、間違いがあった場合、他の参加者の回答の傾向をみて修正した。この作業にそれほど時間はかからなかった。

%次に、全ての参加者の全ての手書き文字とタイプインデータとの照合を行った。この結果、ある程度の打ち間違いがあり、中には回答欄を列ごと間違えている場合も1件あった。これらの齟齬の修正を行ったが、何と書こうとしたのか判断に迷う場合は、修正しなかった。

%この確認と修正には、参加者ひとりあたり20分$\sim$30分要した。今回は30人$\times$2回の規模であったので修正が行えたが、実験規模をさらに大きくする場合は検討が必要である。ただし、以下に述べる今回の分析範囲では、この作業を行わなくても大きく結果は変わらなかった。これは、クラウドソーシング登録者集団の特性(たとえば真面目かどうか)に依存するかもしれない。


%一連の修正作業において、参加者1名(2回の実験両方に参加)が、回答を多数書き直していることを発見した。各回200単語のうち1回目が86単語、2回目が89単語と、他の被験者の書き直し数(ほとんどが数単語未満で、2名ほど30と40)よりも著しく多かった。音声提示からの回答時間は4秒であり、その時点で書き換える余裕はないので、明らかに事後に音声を聞かずに書き変えたと考えられる。このことから、この参加者は実験の意図を理解せず行ったと判断し、以降の分析から除外した。 このことから、まず残りの29名分のタイプインデータから単語完全正答率を計算した。


\begin{figure*}[t]
  \begin{center}
    \begin{tabular}{c}
      % 1
      %\hspace{-5mm}
      \begin{minipage}{0.65\columnwidth}
        \begin{center}
        \hspace{-12mm}
             \includegraphics[width = 1\columnwidth]
    {Figure/Fig_6_InterSp21.eps} 
    \label{fig:Exp1_ResultEval}
          \caption{Speech reception threshold (SRT) in dB. Blue: Remote experiment, Red: Laboratory experiment\SRT}

        \end{center}
      \end{minipage}
    \hspace{7mm}
      % 2
      \begin{minipage}{0.65\columnwidth}
        \begin{center}        
        \hspace{-12mm}
    \includegraphics[width = 1\columnwidth]
    {Figure/Fig_7_InterSp21.eps} 
    \label{fig:Exp1_ResultEval}
          \caption{Speech reception threshold (SRT) in dB. Blue: Remote experiment, Red: Laboratory experiment\SRT}
        \end{center}
      \end{minipage}
    \hspace{7mm}
      % 3
    \end{tabular}
      \end{center}
      \vspace{-25pt}
\end{figure*}

% もっと詳しく、SRTのばらつきを調べるため、参加者の属性とSRTとの関係について一般化線型分析を行った。
% これは、事前にデータを
% apriori and posteriori screening

%今回のWebページ\cite{ExpSpIntel}による実験では、クラウドソーシングサイトで公開されている情報も含めて、参加者のプロフィール情報が得られる。この情報からSRTが予測できるかを検討した。うまくいけば事前のデータ削減にも役立てられる。

%ここでは、29名のデータ``Sbj29''に関し、SRTを目的変数として以下の指標から一般化線形モデル(ここでは手始めに正準リンク関数を用いた)で予測することを試みた。説明変数は、各参加者の\ctext{a}性別\ctext{b}年齢\ctext{c}機材(ヘッドホン/イヤホン)\ctext{d}実験時のIDとクラウドソーシング登録情報の相違から計った信頼性\ctext{e}手書き回答用紙の修正数\ctext{f}タイプインの誤字数\ctext{g}4モーラ修正数\ctext{h}練習問題の正解数（全10問）\ctext{i}実験時間（分）である。２回実験に参加した者の場合、初回の練習問題の正解数（低い成績）を採用した。また、2回の各実験ごとに強調処理条件のSRTの平均を求めた。

%図\ref{fig:GLM_SS}上図に、1回目の実験のSRTと一般化線型モデルで予測されたSRTの散布図を示す。ここで、上記9個全ての説明変数を用いた場合(x)とステップワイズ法で説明変数を削減した場合(o)を示した。両者が一致する対角線(点線)から大きくはずれる点が多い。
%ステップワイズ近似では、

%というモデル式が得られた。図\ref{fig:GLM_SS}下図に練習問題正解数に対する参加者のSRTと、上記の回帰直線を示した。傾向は捉えているが、そもそもばらつきが大きいため、十分な精度は出ない。2回目の実験も同様な結果であった。1回目、2回目の推定標準偏差は1.41と1.58となった。これは、 図\ref{fig:ExpAYama20_Sbj29}の標準偏差より若干小さい程度である。他の指標はSRT予測に有効でないこともわかった。
%このことから、精度は高いとは言えないものの、練習問題正解数はデータ削減の一つの目安となりえることがわかった。



% どのような条件が、remoteをlabに近づけることにつながるかを調べた。
% 　これは、apriori にデータscreeningできれば、信頼性の低いデータを排除し、より良く活用できる可能性があるためである。

% improvement was within the range of variability

% このことはindividual difference of participantsに起因する。
% 結局どのpaticipants も、SRTは異なるものの、同じ傾向の回答をしていることがわかった。


%上記の遠隔実験の29名分のデータを用いた結果では、SRTの平均や標準偏差が防音室実験\cite{Ohashi2018Babble, Iwaki2019Onatsu}より大きいことは否めない。そこで明確な基準を設けて元データを削減することにより、近い結果が得られるかについて検討した。まず、ここでは練習問題正解率に基づいて、分析対象データの選別を行った。\ref{sec:exp_Crowd}節で述べたとおり練習問題で使用したのは最高親密度の単語で、SNRが0\,dB以上である。この場合、通常は間違うことなく聞き取ることが可能だと考えられる。したがって、練習問題の成績が低い参加者は、実験意図の理解不足や書き取りが追いつかない等の問題があり、実験をうまく行えなかった可能性がある。
%さらに、\ref{sec:SRTPrediction}節に述べるように、実験参加者のプロフィールや実験データの分析から、SRTと練習問題正解率との間に相関があることがわかったため、この基準を使うこととした。

% 先行研究とより近い結果を得るために、明確な基準を設けてデータの選別を行った。
%そこで、上記で述べたように各参加者のSRTには練習問題の正解数が関与していることを受けて、
%ここでは、練習問題の正解数が8問以上である参加者を選別した。

%ここでは、練習問題の正解数が8問以上である参加者を選別した。1回目は24名で2回目は26名となった。この結果を分析した結果の心理物理曲線とSRTの平均と標準偏差を、図\ref{fig:ExpAYama_SbjElim8-10}に示す。削減前の図\ref{fig:ExpAYama20_Sbj29}に比べて、心理物理曲線は多少上方にずれたが、差異はほとんど目立たない。SRTで見ると、全ての強調処理条件で平均値が若干減少し、標準偏差も小さくなった。しかし、防音室実験の図\ref{fig:ExpLab_KY17}や図\ref{fig:ExpLabLowSPL_RI18}に大きく近づくわけでもないこともわかった。練習問題の正解数が9問以上である参加者を選別すると（1回目は17名で2回目は22名）、さらに平均値・標準偏差が若干減少するものの、防音室実験結果と一致するまでには至らなかった。



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 



% \{``${\rm WF_{PSM}^{(0.0)}}$'', ``${\rm WF_{PSM}^{(0.2)}}$''\}.

% さらに詳細検討するため、各参加者ごとの了解度データから、語音聴取閾値(SRT, Speech Reception Threshold)を求めた。この際、ベイズ法による心理物理曲線推定手法psignifit\cite{psignifit}を用い、累積ガウス分布をあてはめて50\%となるSNR (dB)値(=SRT)を各参加者・強調処理条件毎に求めた。
% 図\ref{fig:ExpAYama20_Sbj29}下図、図\ref{fig:ExpLab_KY17}下図、図\ref{fig:ExpLabLowSPL_RI18}下図に、それぞれの実験に対応するSRTの参加者間平均と標準偏差を示す。横軸は強調処理条件\{``Unprocessed'', ``SS10'',``VTS00'',``VTS02''\}である。

%%% %図\ref{fig:ExpAYama20_normal}に遠隔実験の参加者29名のSRTの平均を示す。また、\ref{fig:ExpKY17}\ref{fig:ExpRI18}は、先行研究\cite{Ohashi2018Babble}で行われた防音室実験の結果と、先行研究\cite{Iwaki2019Onatsu}の提示音圧低減を行った防音室実験の結果である。それぞれグラフの縦軸はSRT、横軸は信号処理条件、エラーバーは標準偏差を表している。

% 遠隔実験は、2つの防音室実験に対して、全ての強調処理条件においてSRTが高く、標準偏差も大きいことがわかる。特に``Unprocessed''では、お互いの相違が大きい。それ以外の強調処理では、図\ref{fig:ExpLabLowSPL_RI18}の音圧低減実験に似た傾向がある。

% このような相違点があるものの、4つの強調処理条件のSRTの大小関係は同じであることがわかった。

% GEDI\cite{yamamoto2020gedi}等の客観評価指標の開発においては、``Unprocessed''の了解度を用いてパラメータ設定を行い、強調処理条件の了解度がどの程度良く推定できるかで評価される。強調処理条件のSRTの大小関係が同じであることは、遠隔実験結果もいままでの防音室実験結果と同様に利用できることを示唆している。




% CrowdMOSのようにposterioriに処理することが多い。
% しかし、こうすると、実験者の人為的なバイアスの影響を排除できない。
% どこに基準を設けるかも明確ではない。

% aprioriでほぼ同じ結果となるのであれば、こちらの方がbetterであろう。
% しかし、criterionを設けることにより、分析するデータ数が減少するため、注意は必要となるであろう。



% Remote testing using crowd-sourcing would be a good tool to collect massive subjective data if hearing level is not under consideration (??)


% Further studies are neThe SRT prediction using the stepwise approximationwith the generalized linear model extracted the practice score assolely correlated explanatory variable. It seems a good criterionfor data selection although other factors should be investigatedmore.

% このことはindividual difference of participantsに起因する。
% 結局どのpaticipants も、ややSRTの大小はあるものの、同じ傾向の回答をしていることがわかった。
% このため、客観評価指標開発にも有効な手段となろう。
%
% さらに年齢層やその他の要因ごとに被験者特性を測るためには、クラス分けしても十分なmassive dataを集めやすいCrowd-sourcingは有効な手段であることがわかる。
% もっとも、Crowd-sourcingに登録する人間のIT skill は平均的なpopulation よりやや高いかかもしれないが。
% これに関しては、他のパラダイムで検証するしかない。



% The F(difference from  p-value were 0.015 and ** in the first and second remote experiments respectively and they were significantly different from null hypothesis of no correlation. 

% The results imply that the score of practice session is only the factor influencing the SRT values although the prediction errors (1.4\,dB and 1.6 \,dB) were roughly the same as the standard deviations of the SRT and not very small.

%  in Wilkinson notation as 
%    \vspace{-7pt}
%\begin{equation}
%    {\rm SRT (dB)} \sim 1 + {\rm (score\ of\ practice\ session) }.
%    \vspace{-7pt}
%    \label{eq:SPLdB_Vo}
%\end{equation}
%% 数値をチェック。場所が残れば、図面を入れても良い
% T:

==> Previous/testFig.tex <==

%%%%%% comment out
\begin{comment}
%% Figure
\newlength{\subfigwidth}
\newlength{\subfigcolsep}
\setlength{\subfigcolsep}{2\tabcolsep}
\setkeys{Gin}{width=\subfigwidth}
\begin{figure*}[t]
  \setlength{\subfigwidth}{0.5\linewidth}
 % \addtolength{\subfigwidth}{-.5\subfigcolsep}
\begin{tabular}{ccc}
    \hspace{-9mm}
    \begin{minipage}{0.6\subfigwidth}
      \centering
         %\hspace{-8mm}
      \includegraphics[width=1.1\columnwidth]{Figure/Fig_Exp_Lancers_AYama20_Pcorrect_SbjElim_2-30.eps}
      \label{fig:ExpAYama20_Sbj29}
        \vspace{-5mm}
      \caption{Crowd-sourcing remote experiment: Average and standard deviation of word correct (\%) }
      \label{fig:ExpAYama_SbjElim8-10}
    \end{minipage}
   \hspace{3mm}
    \begin{minipage}{0.6\subfigwidth}
      \centering
      %\vspace{-1mm}
      \includegraphics[width=1.1\columnwidth]{Figure/Fig_Exp_Lab_KY17_Pcorrect_Word.eps}
      \vspace{-4mm}       
      \caption{Laboratory experiment: Average and standard deviation of word correct  (\%)  }
      \label{fig:ExpAYama_SbjElim8-10}
    \end{minipage}
     
    \hspace{3mm}
    
    \begin{minipage}{0.6\subfigwidth}
      \centering
      \includegraphics[width=1.1\columnwidth]{Figure/Fig_mCmpr12_SRTdB_bar_xExp+xNsRdct_SbjElim_2-30.eps}
      \caption{Speech reception threshold (SRT) in dB. Blue: Remote experiment, Red: Laboratory experiment\SRT}
      \label{fig:ExpLab_KY17}
    \end{minipage}
     
    \hspace{3mm}
    

\end{tabular}
\end{figure*}


\end{comment}

